A Temporal-Difference Approach to Policy Gradient Estimation

The policy gradient theorem (Sutton et al., 2000) prescribes the usage of a cumulative discounted state distribution under the target policy to approximate the gradient. Most algorithms based on this theorem, in practice, break this assumption, introducing a distribution shift that can cause the convergence to poor solutions. In this paper, we propose a new approach of reconstructing the policy gradient from the start state without requiring a particular sampling strategy. The policy gradient calculation in this form can be simplified in terms of a gradient critic, which can be recursively estimated due to a new Bellman equation of gradients. By using temporal-difference updates of the gradient critic from an off-policy data stream, we develop the first estimator that sidesteps the distribution shift issue in a model-free way. We prove that, under certain realizability conditions, our estimator is unbiased regardless of the sampling strategy. We empirically show that our technique achieves a superior bias-variance trade-off and performance in presence of off-policy samples.

==> figures/imani-mdp.tex <==
\begin{tikzpicture}
	\node (cartpole) at (0,0) {
		\includegraphics[width=0.4 \columnwidth]{figures/imani.pdf}};
	\node [above=-8pt of cartpole.north] {\textsuperscript{(a) Imani's MDP}};
	\node [below=.0cm of cartpole.south] {};
\end{tikzpicture}

==> sections/background.tex <==
\section{Background}
\label{sec:background}
We consider a Markov decision process $\mathcal{M} = <\!\Sset, \Aset, r, P, \mu_0\!>$, where $\Sset$ represents the set of states, $\Aset$ the set of actions, $r:\Sset\times\Aset\to\mathbb{R}$ the reward signal, $P(\state'|\state,\state)$ the probability density of transitioning to state $\state'$ after the application of action $\action$ in state $\state$, and $\mu_0$ the distribution of the starting state.
The policy $\pi_\theta$ is a stochastic mapping with density $\pi_\theta(\action|\state)$ parametrized by a vector $\theta \in \mathbb{R}^{n_p}$ and differentiable w.r.t. it.
We denote with $S_t, A_t, R_t$ the stochastic variables representing the state, action, and reward at time $t$.
The state-distribution $\mu^{\pi}_t(\state)\! =\! p(S_t\!=\! \state)$ indicates the (density of) probability of the state $\state$ being observed at time $t$. The discounted state distribution $\mu^{\pi}_\gamma(\state) = (1-\gamma)\sum_{t=0}^\infty\gamma^t\mu^{\pi}_t(s)$ defines the probability of observing the state $\state$ in any moment, giving a $1-\gamma$ probability of the episode to restart from $\mu_0$ at each time step. We denote with $\mu_\beta(\state)$ the off-policy  state distribution induced by the behavioral policy $\beta$. Let $\tau_\pi \equiv \{(S_t, A_t, R_t)\}_{t=0}^{T_\tau}$ be an on-policy trajectory (where $T_\tau$ denotes trajectory's length, which can also be infinite). Similarly, $\tau_\beta$ represent an off-policy trajectory.
The objective of reinforcement learning is to maximize the expected discounted return 
\begin{align}
	J(\theta) = (1-\gamma)\E_{\tau_\pi}\left[\sum_{t=0}^\infty \gamma^tR_t\right]. \label{eq:return}
\end{align}
The $Q$-function  $Q^\pi(\state, \action) = \mathbb{E}[\sum_{t=0}^\infty R_t| S_0=\state, A_0=\action]$ can be defined recursively as 
\begin{equation}\small
	Q^\pi(\state, \action)\! =\! r(\state, \action)\! + \! \gamma \int_\Sset\int_\Aset Q^\pi(\state', \action')p(\state'|\state, \action)\pi_\theta(\action' | \state')\!\de \action \! \de \state' . \label{eq:bellman}
\end{equation}
The value function $V^\pi(\state) = \int_\Aset Q^\pi(\state, \action)\pi_\theta(\action | \state) \de \action$ determines the expected cumulation of discounted rewards from state $\state$.

\textbf{Policy Gradient Theorem.} One of the most important results in reinforcement learning is the policy gradient theorem (PGT), which states that
\begin{align}
	\nabla_\theta J(\theta) = \underset{\substack{S \sim \mu_{\gamma}^\pi \\ A \sim \pi_\theta}}{\mathbb{E}}\left[Q^{\pi_\theta}(S, A)\nabla_{\theta}\log\pi_{\theta}(A| S)\right]. \label{eq:pgt}
\end{align}
PGT has also been formulated for deterministic policies \citep{silver_deterministic_2014} and for stochastic policies using the reparametrization trick \citep{haarnoja_soft_2018,heess_learning_2015}.
Despite its fundamental importance, PGT does not provide a direct solution for off-policy learning, leaving open the question of how to approximate the gradient by using samples from a different state distribution $\mu_\beta$.{\color{red} insert semi-gradient below}
%Among the many techniques that have been developed to approximate the policy gradient using off-policy samples, we identify two main cathegories that include most of the algorithms: the \textsl{semi-gradients} (SG) like OffPAC, DPG, DDPG, TD3, SAC, and the ones based on \textsl{importance sampling} (IS).
%\\
%\textbf{Semi-Gradient} approaches do not consider the state-distribution shift, and simply compute the gradient as an expectation over $\mu_\beta$, e.g.,
%\begin{align}
%	\hat{\nabla}_{\theta}^{SG} J(\theta) = \underset{\substack{S\sim \mu_\beta \\ A \sim \beta}}{\mathbb{E}}\left[\frac{\pi_\theta(A|S)}{\beta(A|S)}Q^{\pi_\theta}(S, A)\nabla_{\theta}\log\pi_{\theta}(A| S)\right]. \nonumber
%\end{align}
%This approximation introduces an irreducible bias in the gradient estimator (which does not vanish with larger provision of samples). 
%The term \textsl{semi-gradient} has been adopted in the context of gradient estimation by CITE, and recall that this estimator is the result of the omission of a term in the gradient expansion,
%\begin{align}
%	\nabla_\theta V^\pi(\state)\! &  = \!\int_\Aset\! Q^\pi(\state, \action)\nabla_\theta \pi_\theta(\action | \state) \!+\! \pi_\theta(\action | \state) \nabla_\theta Q^\pi(\state, \action) \! \de \action \nonumber  \\ \scriptsize 
%	& \approx  \int_\Aset Q^\pi(\state, \action)\nabla_\theta \pi_\theta(\action | \state) \de \action
%\end{align}
%The popularity of SG comes perhaps from their simplicity, and, despite the biased estimation, they have been shown to converge to the optimal solution in a tabular setting (finite state-space and tabular policy). The convergence guarantee does not hold, however, for continuous states and biased estimates of the critic.

==> sections/bootstrapped-gradient.tex <==
\section{Bootstrapped Policy Gradient}
We rewrite the PGT theorem in terms of a summation of \textsl{immediate-gradient} terms $Q^\pi (\state, \action)\nabla_\theta \log \pi_\theta(\action| \state)$ at different time-steps, plus an additional \textsl{bootstrapped-gradient} term $\nabla_\theta V^\pi(\state)$. 
\begin{proposition}[$n$-Step Bootstrapped Gradient]\label{prop:n-step}
	\begin{equation}\scriptsize
		\nabla_\theta J(\theta)\!  =\!  \underset{\tau_\pi}{\mathbb{E}}\left[ \sum_{t=0}^{T-1} \gamma^t Q^\pi(S_t, A_t)\nabla_\theta \log \pi_\theta(A_t | S_t)\! + \! \gamma^T \nabla_\theta V^\pi(S_t)\right] 
	\end{equation}
	for any $T \geq 1$.
\end{proposition}
This alternative (and equivalent) view highlights a relation to the concept of bootstrapping for PE (Figure~\ref{fig:pe-bpg}). 
In facts, Propositon~\ref{n-step} shows that the gradient can be seen as a Monte-Carlo rollouts of \textsl{immediate}-gradients, plus the bootstrapping terms. Intuitively, for a longer $T$ the variance of the estimate will be larger. We will see later that we are able to approximate $\nabla_\theta V^\pi$ by adding a bias. Therefore, one can trade-off bias and variance by choosing properly the time horizon $T$. This result reminds the bootstrapping in the context of PE, i.e., 
\begin{align}
	J(\theta) = \underset{\tau_\pi}{\mathbb{E}}\left[\sum_{t=0}^{T-1} \gamma^tR_t + \gamma^T V^\pi(S_T)\right]
\end{align} where $V^\pi$ is usually estimated via ADP.
Inspired by the connection with policy evaluation, we define the concept of $\lambda$-gradient, which is the gradient counterpart of eligibility traces. 

Inspired by this connection, we propose an elegibility trace version of the PGT.
\begin{proposition}[$\lambda$-Gradient]\label{prop:lambda-gradient}
	For any $\lambda \in (0, 1]$,
	\begin{align}
		\nabla_\theta J(\theta) = &  \underset{\tau_\pi}{\mathbb{E}}\bigg[\sum_{t=0}^{T_\tau}\lambda^t\gamma^t\big( \lambda Q^\pi(S_t, A_t)\nabla_\theta \log \pi_\theta(A_t | S_t)\nonumber  \\
		& \quad + (1-\lambda) \nabla_\theta V^\pi(S_t)\big)\bigg].
	\end{align}
\end{proposition}
Setting $\lambda \to 0$ allows to consider only the bootstrapped term at the initial state distribution, i.e.,
\begin{align}
	\lim_{\lambda \to 0} \nabla_\theta J(\theta)  = \underset{\mu_0}{\mathbb{E}}\left[\nabla_\theta V^\pi(S) \right],
\end{align}
conversely, when $\lambda \to 1$ one considers the summation of all immediate-gradients,
\begin{align}
	\lim_{\lambda \to 1} \nabla_\theta J(\theta)  = \underset{\tau_\pi}{\mathbb{E}}\left[\sum_{t=0}^{T_\tau}\gamma^t Q^\pi(S_t, A_t)\nabla_\theta \log \pi_\theta(A_t | S_t)\right].
\end{align}
In other words, when $\lambda$ is low, the estimator tends to consider a shorter horizon and to give higher importance to the bootstrapping term, while when $\lambda$ is higher, the estimator tends to consider a longer horizon and give higher importance to the immediate term.

==> sections/bootstrapped-objective.tex <==
\section{A Bootstrapped Objective}


==> sections/bpg.tex <==

\section{Estimating the Gradient Function}
When we look at the return in Equation~\ref{eq:return}, we see that it is composed by a summation of rewards that depends on on-policy trajectories. Using action value functions, however, we can rewrite the return only in terms of the starting state distribution, i.e., 
\begin{align}
	J(\theta) = (1-\gamma)\mathbb{E}_{\mu_0, \pi_\theta}\!\left[Q^\pi(\state, \action)\right]. \label{eq:return1}
\end{align}
The $Q$-function can be approximated via off-policy samples, allowing, therefore, the return to be fully described using off-policy samples.
Similarly, the PGT can be seen as a summation of ``immediate'' terms\footnote{Trough the paper, we switch from trajectory-based (using $\mathbb{E}_\tau$) PGT to discounted state-distribution based PGT (using $\mathbb{E}_{\mu^\pi_\gamma}$) according to the need. The two formulations are equivalent up to a proportional factor $1-\gamma$.}
\begin{align}
	\nabla_\theta J(\theta) \propto \mathbb{E}_\tau\!\Bigg[\sum_{t=0}^\infty\gamma^t\underbrace{Q^\pi(S_t,\! A_t)\nabla_\theta\! \log\! \pi_\theta(A_t|S_t)}_\text{immediate gradient}\Bigg], \nonumber 
\end{align}
reminding of Monte-Carlo rollouts used in policy evaluation (Figure~\ref{fig:monte-carlo}). Inspired by this connection, we want to work out a recursive definition of the policy gradient that requires only sampling the starting state distribution. We can do that by differentiating on both the sides Equation~\ref{eq:return1},
\begin{align}
	\nabla_\theta J(\theta) =&  (1-\gamma) \int_\Sset \int_\Aset \mu_0(\state )\left(\nabla_\theta Q^\pi(\state, \action)\right)\pi_\theta(\action | \state) \nonumber \\
	& + \mu_0(s) Q^\pi(\state, \action)\nabla_\theta\pi_\theta(\action |\state)\de \action \de \state . \label{eq:first-derivation}
\end{align}
In Equation~\ref{eq:first-derivation}, the term $\nabla_\theta Q^\pi(\state, \action)$ is usually unknown. Predicting $\nabla_\theta Q^\pi(\state, \action)$ potentially overcomes the need of the on-policy discounted distribution $\mu_\gamma^\pi$, as allows the gradient estimation to rely solely on the starting-state distribution $\mu_0$.\\
\textbf{Gradient Function.} The focus of this paper is to approximate the gradient function $\bm{\Gamma}^\pi(\state, \action) = \nabla_\theta Q^\pi(\state, \action)$ using off-policy samples.
The gradient-function $\bm{\Gamma}:\Sset\times\Aset\to\mathbf{R}^{n_p}$ can be defined by differentiating on both the sides the Bellman equation in \eqref{eq:bellman} and substituting $\nabla_\theta Q^\pi(\state, \action)$ with $\bm{\Gamma}^\pi(\state, \action)$, 
\begin{align}
	\bm{\Gamma}^\pi(\state, \action)=&\gamma\int_\Sset\int_\Aset\Big( Q^\pi(\state', \action')\nabla_\theta\log\pi_\theta(\action'|\state') \nonumber  \\
	& + \bm{\Gamma}^\pi(\state', \action')\Big)\pi(\action'|\state')p(\state'|\state,\action)\de \action'\! \de \state'. \label{eq:gradient-bellman}
\end{align}
We call Equation~\ref{eq:gradient-bellman} \textsl{gradient Bellman equation}.
%both as a cumulations of \textsl{immediate gradients}, 
%\begin{equation}\resizebox{\columnwidth}{!}{$
%	\bm{\Gamma}^\pi(\state, \! \action)\! = \!\mathbb{E}\!\left[\sum_{t=1}^\infty\gamma^tQ^\pi(S_t,\! A_t)\nabla_\theta\! \log\! \pi_\theta(A_t|S_t) \bigg| S_0\!=\!\state,\! A_0\! =\! \action\right]\! , \nonumber $}
%\end{equation}
%or recursively in terms of a \textsl{gradient Bellman equation}.
%Equation~\ref{eq:gradient-bellman} can be derived taking the gradient on both the side of Equation~\ref{eq:bellman}. 
\begin{figure}[t]
%	\includegraphics[width=\columnwidth]{figures/gradient-function.pdf}
	\input{figures/reward-flow.tex}
	\input{figures/gradient-flow.tex}
	\caption{Likewise the return, the policy gradient can be seen as the cumulation of \textsl{immediate} terms. A parametric approximation of the policy gradient avoids the need of an on-policy sampling process.\label{fig:monte-carlo}}
\end{figure}
It is possible to see that Equation~\ref{eq:gradient-bellman} is a proper Bellman equation. In fact, \eqref{eq:gradient-bellman}  can be seen as a set of indipendent scalar Bellman equations
\begin{align}
	\Gamma^\pi_i(\state, \action)=& \iota_i(\state, \action)  + \gamma\! \int \! \Gamma^\pi_i(\state', \action')\pi(\action'|\state')p(\state'|\state,\action)\! \de \action'\! \de \state' \nonumber 
\end{align}
with average ``reward signal'' 
\begin{align}
	\iota_i(\state, \action) = \gamma\int_\Sset\int_\Aset  Q^\pi(\state', \action')\frac{\partial}{\partial \theta_i} \pi(\action'|\state')p(\state'|\state,\action)\de \action'\! \de \state'. \nonumber % \label{eq:immediate-gradient}
\end{align}
Bellman equations are well studied, giving us access to a broad literature about approximation techniques and theoretical results. In the following, we focus mainly on how to approximate the gradient function using temporal difference methods. 

==> sections/eligibility-traces.tex <==
\section{Eligibility Traces Policy Gradient}
Our approach has the benefit of having low bias under off-policy distribution (when the features are good enough to represent the critic, Theorems~\ref{theo:GLS}~and~\ref{theo:perfect-features}), however, such benefit is questionable since: 1) learning $\bm{\Gamma}^\pi$ online can causes delays in the gradient estimation that potentially hinder the benefit of a lower bias\footnote{A similar delay happens between classic actor and critic estimators.} 2) the gradient function is learned under the off-policy distribution but is used only under the starting-state distribution 3) the starting states are usually sampled rarely, potentially disallowing a frequent gradient update.s

A way to overcome the mentioned problems is to interpolate the two algorithms. Inspired by the parallel between the PGT and the Monte-Carlo rollouts discussed in Section~\ref{sec:background}, we provide a $n$-step version of the PGT
\begin{align}
	\nabla_\theta J(\theta) \propto &\underset{\tau_\pi}{\mathbb{E}}\bigg[\sum_{t=0}^{T-1} \gamma^{t}Q^\pi(S_t, A_t)\nabla_\theta \log \pi_\theta(A_t|S_t) \nonumber  \\
	& \quad+ \gamma^{T-1}\bm{\Gamma}^\pi(S_{T-1}, A_{T-1})\bigg] \label{eq:n-step-gradient}
\end{align}
From the $n$-step view is almost trivial to extend the PGT to eligibility traces (details in Appendix~\ref{app:eligibility-trace}),
\begin{align}
	\nabla_\theta J(\theta) \propto &  \underset{\tau_\pi}{\mathbb{E}}\bigg[\sum_{t=0}^{\infty}\lambda^t\gamma^t\big(Q^\pi(S_t, A_t)\nabla_\theta \log \pi_\theta(A_t | S_t)\nonumber  \\
	& \quad + (1-\lambda) \bm{\Gamma}^\pi(S_t, A_t)\big)\bigg]. \nonumber 
\end{align}
Notice that with $\lambda=0$, one can recover the policy gradient scheme introduced earlier in Section~\ref{sec:background} (since $\lim_{\lambda\to 0}\lambda^0=1$), where all the contribution is given by $\bm{\Gamma}$ at the starting state distribution, and $\lambda\to 1$ recovering the classic PGT. However, in this paper, we are interested in estimating the gradient using off-policy data. One possiblity would be to correct the off-policy distribution with ``path-wise'' importance sampling corrections. In that case $\lambda$ will trade-off the high variance of a full importance sampling approach, and the bias of our gradient estimator,
\begin{align}
	\nabla_\theta J(\theta) \propto &  \underset{\tau_\beta}{\mathbb{E}}\bigg[\sum_{t=0}^{\infty}\lambda^t\gamma^t\rho_t\big(Q^\pi(S_t, A_t^\pi)\nabla_\theta \log \pi_\theta(A_t^\pi | S_t)\nonumber  \\
	& \quad + (1-\lambda) \bm{\Gamma}^\pi(S_t, A_t^\pi)\big)\bigg], \nonumber
\end{align}
where $\rho_0 = 1$, $\rho_t = \prod_{i=0}^{t-1} \pi(A_i |S_i)/\beta(A_i | S_i)$, $\tau_\beta$ are off-policy trajectories and $A_t^\pi \sim \pi_\theta(\cdot | S_t)$ are on-policy actions (used to reduce the gradient's variance).
Alternatively, we omit the importance sampling correction, offering a way to blend the semi-gradient with our approach,
\begin{align}
	\nabla_\theta J(\theta) \approx &  \underset{\tau_\beta}{\mathbb{E}}\bigg[\sum_{t=0}^{\infty}\lambda^t\gamma^t\big(Q^\pi(S_t, A_t^\pi)\nabla_\theta \log \pi_\theta(A_t^\pi | S_t)\nonumber  \\
	& \quad + (1-\lambda) \bm{\Gamma}^\pi(S_t,A_t^\pi)\big)\bigg]. \label{eq:semi-traces}
\end{align}
Algorithm~\ref{alg:tdc-gamma} describes a possible policy-improvement by estimating the gradient funcion with $\bm\Gamma$RC and using it with eligibility traces as in \eqref{eq:semi-traces}.
Of course, the gradient function can be estimated and used in many different ways. To allow simple theoretical analysis and convergence properties, we considered only linear gradient functions and specific temporal difference algorithms. Nothing prevents the exploration of non-linear approximators, replay buffers, and the combination our gradient estimator with more sophisticated approaches. 


==> sections/introduction.tex <==
\section{Introduction}
\begin{figure}[t]
	\centering
	\input{figures/actor-critic.tex}
	\input{figures/gradient-actor-critic.tex}
	\caption{(a) Classic actor-critic scheme.  (b) We introduce a functional approximation of the policy gradient in the pipeline.\label{fig:gradient-actor-critic}}
\end{figure}
In the recent years, policy gradient methods gained popularity in the reinforcement learning community \citep{haarnoja_soft_2018,schulman_trust_2015, schulman_proximal_2017,lillicrap_continuous_2016}. Their robustness, sample efficiency, and ability to deal with continuous action spaces (as well as discrete ones) make them suitable for a large variety of applications, from computer games \citep{vinyals_grandmaster_2019}, robotics \citep{haarnoja_soft_2018,mahmood_setting_2018}, and, in general, real-world applications.

Reinforcement learning algorithms aim to maximize the expected cumulation of rewards during the agent's interaction with the environment.
Policy gradient methods estimate the gradient of this objective w.r.t. the policy's parameters.
One of the most important results in this field is the policy gradient theorem (PGT) \cite{sutton_policy_2000}, which provides a formula for computing the policy gradient in terms of an expectation under the discounted on-policy state distribution. Such condition is generally restrictive, since it disallow sample reuse from past policies. 

Off-policy estimation, a common technique for sample reuse, can also be used for policy gradients by adopting some countermeasures. One way is to use importance sampling to correct the distribution shift induced by the off-policy distribution \citep{meuleau_exploration_1999,shelton_policy_2001,peshkin_learning_2002,metelli_policy_2018,liu_off-policy_2019}. These techniques usually suffer from high variance estimation. Furthermore, they require 1) temporal-ordered stream of data and 2) knowledge of the behavioral policy, as discussed in \cite{tosatto_batch_2020}. In some cases, the temporal order is not available (can happen in offline reinforcement learning), in others, the importance sampling is not computable due to the numerical unavailability of behavioral policy, or from some other source of distribution mismatch, such as premature episode termination.

A more popular way to deal with off-policy samples in the context of policy gradient is to neglect the distribution correction. This approach, which we call \textsl{semi-gradient} \citep{imani_off-policy_2018}, adds a bias to the gradient estimation. \cite{imani_off-policy_2018} show that this bias can cause convergence to poor solutions even in simple three states problems. Semi-gradient approaches, like OffPAC \citep{degris_off-policy_2012}, DDPG \citep{lillicrap_continuous_2016}, A3C \citep{mnih_asynchronous_2016}, TD3 \citep{fujimoto_addressing_2018} and SAC \citep{haarnoja_soft_2018}, work with a mild distribution shift induced by the replay buffer. \cite{fujimoto_off-policy_2019} suggests that the effectiveness of aforementioned approaches can be hindered when the distribution shift is more pronounced.

%Several works go in the direction of mitigating the high-variance of full importance sampling correction \citep{imani_off-policy_2018,metelli_policy_2018,liu_off-policy_2019}. Recent work focuses on a modified objective that allows a bi-level optimization that implicitly corrects the off-policy distribution \citep{nachum_algaedice:_2019,nachum_reinforcement_2020}.

Off-policy estimation is not new in the context of reinforcement learning, and in particular, has been deeply analyzed in policy evaluation \cite{XXX}. 
Techniques based on temporal difference allow critic estimation without requiring importance sampling \citep{lagoudakis_least-squares_2003,ghiassian_gradient_2020}. The whole idea of temporal difference is to obtain a parametric estimate of the critic for each state-action pair, so as to overcome the need for rollouts that require sampling from the on-policy distribution. 
In a way similar to policy evaluation, one can avoid the need for the on-policy distribution by approximating the policy gradient with a parametric function. However, such an approach does not exist.

In this work, we propose using temporal difference techniques to approximate the policy gradient. We define a function that returns the full policy gradient from each state-action pairs, which can be seen as a fixed point of a \textsl{gradient Bellman equation}. We call it \textsl{gradient function} and, likewise the value function, it can be approximated using standard temporal-difference techniques.
Our approach, does not require importance sampling. Once estimated, one can query the gradient function on the initial state to recover the full policy gradient, thus overcoming the need for the on-policy distribution.

To work out a theoretical analysis, we assume the gradient function to be linear w.r.t.\ a set of features. We show that in some situation our estimator is unbiased, whereas the \textsl{semi-gradient} remains biased. This advantage helps in recovering from the failures discussed by \cite{imani_off-policy_2018}. The advantegs given by the gradient function can be hindered by the complexity of its practical estimation. To address this issue, we also introduce an approach based on eligibility traces that allows blending the classic semi-gradients with our gradient-function.

We show that, in practice, our approach overcomes the weaknesses of semi-gradient, being still competitive also in scenarios where the semi-gradient performs well.

==> sections/offline-bpg.tex <==
\subsection{A Linear Gradient Function}
Linear architectures coupled with least-squares temporal differences are perhaps the most studied, given their relative simplicity. In this section, we study a least-square temporal difference solution of the gradient function, utilizing a linear function approximator. 
\begin{assumption}[Linear Gradien Function]\label{ass:linear-gradient}
	Let us consider a set of features $\phivec:\Sset\times\Aset \to \mathbb{R}^{n_f}$ and a parameter matrix $\mathbf{G} \in \mathbb{R}^{n_f \times n_p}$. The linear gradient function is defined as
	\begin{align}
		\hat{\bm{\Gamma}}(\state, \action ) = \phivec^\intercal(\state, \action)\mathbf{G}. \nonumber
	\end{align}
\end{assumption}
The fixed point of Equation~\ref{eq:gradient-bellman} can be approximated using the so-called ``least squares'' solution, which can be seen as the fixed point of the projected Bellman operator \citep{lagoudakis_least-squares_2003}. {\color{red} Andrew, do you want to add some comment based on your recent work?}
\begin{lemma}[Least Square Gradient with Perfect Critic]\label{lemma:tdq}
		Let us consider finite state and action sets. For an irreducible Markov chain induced jontly by the transition function $p$ and the policy $\pi_\theta$ having steady distribution $\mu$. Let $\zeta$ be a process where $S \sim \mu_\beta$, $A \sim \beta(\cdot | S)$, $S' \sim p(S' |S, A)$ and $A' \sim \pi_\theta(\cdot |S')$. The least-squares solution of the projected Bellman equation induced by \eqref{eq:gradient-bellman} is 
	\begin{align}
		\hat{\bm{\Gamma}}_{T\!D\!Q}^\pi(\state, \action) = \phivec^\intercal(\state, \action)\mathbf{G}_{T\!D\!Q} \nonumber
	\end{align}
	where $\mathbf{G}_{T\!D\!Q} = \mathbf{A}_\pi^{-1}\mathbf{B}$ and
	\begin{align}
		\mathbf{A}_{\pi} &= \mathbb{E}_{\zeta}\left[\phi(S, A)\left(\phi^\intercal(S, A) - \gamma\phi^\intercal(S', A')\right)\right] \nonumber\\
		\mathbf{B}_Q & = \gamma \mathbb{E}_\zeta\left[\phi(S, A)Q^\pi(S', A')\nabla_\theta \log\pi_\theta(A'|S')\right]. \label{eq:a-b-first}
	\end{align}
	If $p(S, A)$ satisfies the inequality introduced by \cite{kolter_fixed_2011}, then 
	\begin{align}
		& \| \hat{\bm{\Gamma}}^\pi_{T\!D\!Q}(\state, \action) - \nabla_\theta Q^\pi(\state, \action)\|_{\zeta} \leq \nonumber \\
		&\frac{1 + \kappa \gamma}{1-\gamma} \min_{\mathbf{G}}\left\|\phivec^\intercal(\state,\action)\mathbf{G} - \nabla_\theta Q^\pi(\state, \action)\right\|_{\zeta}.
	\end{align}
	with  $\kappa\! =\! \max_{\state, \action}h(\state, \action)/\min_{\state,\action} h(\state, \action)$ where $ h(\state, \action) = \sqrt{\mu(\state)\pi_\theta(\action|\state)}/\sqrt{\mu_\beta(\state)\beta(\action|\state))}$.
\end{lemma}
The result in Lemma~\ref{lemma:tdq} is interesting for two motivations: it gives \textsl{almost} a practical algorithm to estimate the gradient function and obeys the usual least-squares error bound. A practical algorithm consists in estimating $\mathbf{A}_\pi$ and $\mathbf{B}_Q$ via samples. However, $\mathbf{B}_Q$ requires the knowledge of $Q^\pi$. Most algorithms infer the $Q$-function via approximate dynamic programming techniques. To keep our theory consistent, we assume a linear architecture of the $Q$-function approximator.
\begin{assumption}[Linear Critic]\label{ass:linear}
	Consider the set of features in Assumption~\ref{ass:linear-gradient} and a parameter vector $\omegavec \in \mathbb{R}^{n_f}$. The critic is encoded as  $\hat{Q}(\state, \action) = \phivec^\intercal (\state, \action)  \omegavec$.
\end{assumption}
The least squares solution of the classic Bellman equation \eqref{eq:bellman} has sparameters $\omegavec_{T\!D} = \mathbf{A}^{-1}_{\pi_\theta}\mathbf{b}$, with $\mathbf{A}_\pi$ as in Lemma~\ref{lemma:tdq} and $\mathbf{b}  = \mathbb{E}_\zeta[\phi(S, A)r(S, A)]$. 
We replace, therefore, $Q^\pi$ with $\hat{Q}_{T\!D}^\pi$ in Equation~\ref{eq:gradient-bellman},  
\begin{align}
	\hat{\bm{\Gamma}}^\pi(\state, \action)=&\gamma\int_\Sset\int_\Aset\Big( \hat{Q}_{T\!D}^\pi(\state', \action')\nabla_\theta\log\pi_\theta(\action'|\state') \nonumber  \\
	& + \hat{\bm{\Gamma}}^\pi(\state', \action')\Big)\pi(\action'|\state')p(\state'|\state,\action)\de \action'\! \de \state' \label{eq:approx-gradient-bellman}
\end{align}
obtaining the least squares solution 
\begin{align}
	\hat{\bm{\Gamma}}_{T\!D}^\pi(\state,\action) = \phivec^\intercal(\state, \action) \mathbf{G}_{T\!D} \; \text{where}\; \mathbf{G}_{T\!D} = \mathbf{A}_\pi^{-1}\mathbf{B}, \label{eq:gradient-td}
\end{align}
$\mathbf{B}  = \gamma \mathbb{E}_\zeta[\phi(S, A)\hat{Q}^\pi_{T\!D}(S', A')\nabla_\theta\log\pi_\theta(A'|S')]$, and $\mathbf{A}_{\pi}$ as defined in Lemma~\ref{lemma:tdq}.

We can now define a least squares temporal difference approach to $\bm{\Gamma}$ estimation (LSTD$\bm{\Gamma}$) by building a sample estimates of $\mathbf{A}_\pi$ and $\mathbf{B}$. LSTD$\bm{\Gamma}$ can be used to improve the policy (Algorithm~\ref{alg:lstd-gamma}).
Before proceeding with an error analysis of $\bm{\Gamma}_{T\!D}^\pi$, it is worth noting that $\bm{\Gamma}_{T\!D}^\pi$ is the gradient of the least square solution of the critic.
\begin{lemma}\label{lemma:gradient-td}
	The gradient approximation $\hat{\bm{\Gamma}}_{T\!D}^\pi(\state,\action) $ and the least-square critic $\hat{Q}^\pi_{T\!D}(\state,\action)$ satisfy
	\begin{align}
		\hat{\bm{\Gamma}}^\pi_{T\!D}(\state, \action) = \nabla_\theta \hat{Q}^\pi_{T\!D}(\state, \action) \tag*{$\forall \state \in \Sset \land \action \in \Aset$.}
	\end{align}
\end{lemma}
\begin{proof} Consider $\nabla_\theta \hat{Q}^\pi_{T\!D}(\state, \action) = \phivec^\intercal(\state, \action)\nabla_\theta \omegavec_{T\!D}$ and
	\begin{align}
		& \nabla_\theta\omegavec_{TD} = - \mathbf{A}_{\pi}^{-1} 
		\left(\nabla_\theta\mathbf{A}_{\pi}\right)
		\mathbf{A}_{\pi}^{-1} \mathbf{b} \nonumber  \\
		&= - \mathbf{A}_{\pi}^{-1} 
		\left(\nabla_\theta \mathbf{A}_{\pi}\right)
		\omegavec_{TD}\nonumber  \\
		& = \gamma \mathbf{A}_\pi^{-1}\mathbb{E}_\zeta\left[\phivec(S, A)\phivec^\intercal(S', A')\omegavec_{TD}\nabla_\theta \log \pi_\theta(A' | S')\right]\nonumber  \\
		&=  \gamma \mathbf{A}_\pi^{-1}\mathbb{E}_\zeta\bigg[\phivec(S, A) \hat{Q}^\pi_{\mu_\beta}(S', A') \nabla_\theta \log \pi_\theta(A' | S')\bigg].\nonumber \\
		&=  \mathbf{A}_\pi^{-1}\mathbf{B} = \mathbf{G}_{T\!D},\nonumber 
	\end{align}
	implying $\nabla_\theta \hat{Q}^\pi_{T\!D}(\state, \action) =\phivec^\intercal(\state, \action)\mathbf{G}_{T\!D} = \hat{\bm{\Gamma}}^\pi_{T\!D}(\state, \action)$.
\end{proof}
Lemma~\ref{lemma:gradient-td} introduces an interesting connection between our proposed least-square solution of the gradient approximator and the usual least squares solution of the critic. Furthermore, Lemma~\ref{lemma:gradient-td} will be the core of the two following main results. 
\begin{theorem}[Error Analysis]\label{theo:GLS}
	Consider the assumption in Lemma~\ref{lemma:tdq} and Proposition~\ref{prop:generalized-ls}. The least squares approximation $\hat{\bm{\Gamma}}_{T\!D}^\pi$  of the gradient function defined in Equation~\ref{eq:gradient-td} satisfies
	\begin{align}
		&\|\hat{\bm{\Gamma}}^\pi_{T\!D}(\state, \action) - \nabla_\theta Q^\pi(\state, \action)\|_{\zeta} \leq \nonumber \\
		&\frac{1 + \gamma\kappa}{1-\gamma} \min_{\mathbf{G}}\left\|\phivec^\intercal(\state,\action)\mathbf{G} - \nabla_\theta Q^\pi(\state, \action)\right\|_{\zeta} + \nonumber \\
		& \gamma n_p b \kappa \frac{(1+\gamma\kappa)^2}{(1-\gamma)^2}\min_{\omegavec}\|\phivec^\intercal(\state,\action)\omegavec - Q^\pi(\state,\action)\|_{\zeta} \nonumber 
	\end{align}
	with $b = | \max_{\action, \state, i} \partial/\partial\theta_i\log\pi(\action|\state)|$, $n_p$ the number of the policy's parameters  and $\kappa$ as in Lemma~\ref{lemma:tdq}.
\end{theorem}
%
%The TD-solution can be found by LSTD \citep{boyan_least-squares_1999}, but that requires a high amount of computation and storage of large matrixes. Simple online solutions like
%off-policy TD are not guaranteed to converge \cite{baird_residual_1995}. GTD, GTD2, and TDC converge under off-policy data and linear function approximation \citep{sutton_convergent_2008,sutton_fast_2009}, hence $\omegavec_{T\!D}$ can be found using practical algorithms. In the reminder of the paper, we will consider TDC thanks to its convergence guarantee and its computational efficiency.
%
%It is interesting to notice that, by setting proper assumption on smoothness of the feature space, transition distribution and policy, $\omegavec_{TD}$ result differentiable w.r.t. the policy parameters. In particular, knowing that $\de/\de x  \mathbf{M}^{-1}(x) = -\mathbf{M}^{-1}(x)(\de/\de x  \mathbf{M}(x)) \mathbf{M}^{-1}(x)$ where $\mathbf{M}(x)$ is a matrix that depends on a scalar $x$, we are able to compute $\nabla_\theta \hat{Q}_{T\!D}(\state, \action)$ in closed form.
%\begin{proposition}[Gradient of the TD Solution] \label{prop:closed-form}
%	Given the matrix $\mathbf{A}_\pi$ and the vector $\mathbf{b}$ introduced in \eqref{eq:a-b}, and assuming $\mathbf{A}_\pi$  being invertible and differentiable w.r.t. $\theta$,  
%	\begin{align}
%		\frac{\partial}{\partial \theta_i} \omegavec_{TD} = - \mathbf{A}_{\pi}^{-1} 
%		\left(\frac{\partial}{\partial \theta_i}\mathbf{A}_{\pi}\right)
%		\mathbf{A}_{\pi}^{-1}  \mathbf{b}\label{eq:closed_gradient}
%	\end{align}
%	where 
%	\begin{align}
%		\frac{\partial}{\partial \theta_i} \mathbf{A}_{\pi} = -\gamma \mathbb{E}_\zeta \left[\phivec(S, A)\phivec^\intercal(S', A') \frac{\partial}{\partial \theta_i} \log \pi_\theta(A' | S')\right]. \nonumber
%	\end{align}
%\end{proposition}
%Proposition~\ref{prop:closed-form} gives us a simple way to estimate the gradient: one can sample state, actions, reward and next state transition to estimate $\mathbf{A}^\pi$ and $\mathbf{b}$. In other words, we can define a LSTD algorithm to estimate $\nabla_\theta \omegavec_{T\!D}$. We call this algorithm LSTD$\bm{\Gamma}$, and its computation is summarized in lines 2, 4 and 5 of Algorithm~\ref{alg:lstd-gamma} We can now define an approximation of the $\Gamma$-function, 
%\begin{definition}[Temporal-Difference Solution of the Gradient]
%	\begin{align}
%		\hat{\Gamma}_{T\!D}^\pi(\state, \action) = \phivec^\intercal(\state, \action) \mathbf{G}_{T\!D}\label{eq:gamma-td-solution}
%	\end{align}
%where $\mathbf{G}_{T\!D} = \nabla_\theta \omegavec_{T\!D}$.
%\end{definition}
%We are interested to understand \textsl{how good}, in terms of mean squared error, $\bm{\Gamma}_{T\!D}^\pi$ is. By a simple algebraic manipulation of Equation~\ref{eq:offline-policy-gradient}, we notice that $\bm{\Gamma}_{T\!D}^\pi$ is itself a least-squares solution.
Proof in Theorem~\ref{theo:GLS} is relies on the results in \citep{kolter_fixed_2011} and on Lemma~\ref{lemma:gradient-td}. Further details on the proofs can be found in Appendix~\ref{app:least-squares-gradient}. The result relates the projection error of the gradient $\nabla_\theta Q^\pi(\state, \action)$ in the feature space, and, the projection error given by the critic approximation. In other words, the quality of the feature space plays a fundamental role, and when the features are such that these projection error are zero, then $\hat{\bm{\Gamma}}^\pi_{T\!D}(\state, \action) = \nabla_\theta Q^\pi(\state, \action)$. However, the two projection errors defined in Theorem~\ref{theo:GLS} are related, and, surprisingly, it is sufficient to require that $\min_{\omegavec}\left\|\phivec^\intercal(\state,\action)\omegavec - Q^\pi(\state, \action)\right\|_\zeta=0$ to obain a perfect estimate.
\begin{theorem}[Perfect Features]\label{theo:perfect-features} Let $\Phi \equiv \{\phi(\state, \action)  | \forall \state \in \Sset \land \action \in \Aset\}$ and  $\Phi' \equiv \{\phi(\state, \action) - \gamma \int_\Sset\int_\Aset \phi(\state', \action')\pi_\theta(\action'|\state)p(\state'|\state, \action)\de \state\de \action | \forall \state \in \Sset \land \action \in \Aset\}$ be $n_f$-dimensional vector spaces (they both admit at least one basis of dimension $d_f$). Let $\mu_\beta$ be such that $\mathbf{A}_\pi$ is invertible. If we assume that for any policy parameter $\theta$ exists a parameter $\omegavec_\pi$ such that
	\begin{align}
		\phivec^\intercal(\state, \action)\omegavec_\pi = Q^\pi(\state, \action) \tag*{$\forall \state \in \Sset \land \action \in \Aset$,}
	\end{align}
	then
	\begin{align}
		\hat{\bm{\Gamma}}_{T\!D}^\pi(\state, \action) = \nabla_\theta Q^\pi(\state, \action) \tag*{$\forall \state \in \Sset \land \action \in \Aset$.}
	\end{align}
\end{theorem} 
The proof can be found in Appendix~\ref{app:perfect-features}. Theorem~\ref{theo:perfect-features} is particularly important when considering that semi-gradient approaches remain biased even with the knowledge of a perfect critic \citep{imani_off-policy_2018}. 
Notice that Theorem~\ref{theo:perfect-features} allows continuous action space enabling, therefore, the reparametrization gradient \citep{lan_model-free_2021}, as is explained in Appendix~\ref{app:reparametrization}.
%Notice that Theorem~\ref{theo:offline-BPG-perfect} is not a direct consequence of Theorem~\ref{theo:GLS}.
The least square gradient in Proposition~\ref{prop:td} and \ref{eq:first-derivation} allow us to build a policy gradient estimator based on the starting-state distribution,
\begin{align}
	\nabla_\theta \hat{J}(\theta)\! \propto\! \underset{\substack{S \sim \mu_0\\
	A \sim \pi_\theta}}{\mathbb{E}}\big[\hat{Q}_{T\!D}^\pi(S, A)\nabla_\theta \log\pi_\theta(A | S) \!+\! \hat{\bm{\Gamma}}^\pi_{T\!D}(S, A)\big],\label{eq:offline-policy-gradient}
\end{align}
which is unbiased under the assumptions of Theorem~\ref{theo:perfect-features}.
Algorithm~\ref{alg:lstd-gamma} introduces a simple policy improvement scheme based on LSTD$\bm{\Gamma}$. %\sout{One can improve the gradient estimation by introducing a regularization term $\varepsilon \mathbf{I}$ to stabilize the matrix inversion, and using the Sherman-Morrison formula to compute the inversion recursively, as in LSTD$Q$} \citep{lagoudakis_least-squares_2003}. 
 \begin{algorithm}[t]
 	\caption{Policy Gradient with LSTD$\bm{\Gamma}$ \label{alg:lstd-gamma}} 
 	\begin{algorithmic}[1]
 		\State \textbf{Input:} Set of features $\phi$, dataset $D$ of transitions $(\state_i, \action_i, r_i, \state_{i}' )$ where $r_i$ are the rewards and $\state_i'$ the next states, policy $\pi_\theta$, initial distribution $\mu_0$
 		\State {$\hat{\mathbf{b}} =1/N \sum_i \phi(\state_i, \action_i) r_i$}
 		\While {not converged}
 		\State {$\hat{\mathbf{A}} = 1/N \sum_i \phi(\state_i, \action_i)\left((\state_i, \action_i) - \gamma \phi(\state_i', \pi_\theta(\state_i'))\right)^\intercal$}
 		\State {Compute $\mathbf{G}_{T\!D}$ according to \eqref{eq:closed_gradient}}
 		\State {Update $\theta$ according to the gradient in \eqref{eq:offline-policy-gradient}} using samples $\state_0 \sim \mu_0$
 		\EndWhile
 	\end{algorithmic} 
 \end{algorithm}

==> sections/pgt.tex <==
\section{The Difficulty of Sampling from $\mu_\gamma^\pi$}
\label{sec:distribution-shifted}
The PGT asserts that the gradient of the return \eqref{eq:return} w.r.t. the policy parameters is equivalent to the expectation of $Q^\pi(S, A)\nabla_\theta\log_\pi(A | S)$ under the on-policy discounted distribution $\mu_\gamma^\pi$. Practical implementations of several algorithms, however, compute the expectation under a different distribution, adding a bias to the gradient estimation.
\textbf{Off-Policy.} A first approximation is to use the behavioral policy distribution in place of $\mu_\pi$. This approximation happens whenever the policy behaving with the environment is different from the optimization policy (e.g., DDPG uses a stochastic policy on the environment but optimizes a deterministic one). In many offline algorithms, the dataset is collected beforehand. This issue also happens to all those algorithms that use a replay buffer since the replay buffer contains samples obtained with past policies.\\
\textbf{Improper Discounting.} The discounted distribution $\mu_\pi(\state) = (1-\gamma)\sum_{t=0}^\infty\gamma^t\mu^{\pi}_t(s)$  discounts future states. This discounting is, however, not taken in consideration by most of the state-of-the-art techniques, as highlighted by \cite{nota_is_2019}. Uncorrect discounting can be seen as a modification of the discounted state-distribution, and therefore as a source of off-policy data. \\
\textbf{Episode Truncation.} Continuing tasks are designed to have infinite episodes. However, it is impossible to sample infinite episodes in practical scenarios, requiring us to terminate them prematurely. This premature termination also modifies the on-policy distribution, adding a further bias to the gradient estimation.

A na\"{i}ve way to overcome the problem of working with off-policy data, would be to use importance sampling \cite{shelton_policy_2001,meuleau_exploration_2001,peshkin_learning_2002}. However, importance sampling results in high variance estimates, and it is not always applicable. In fact one needs to know the off-policy distribution, but sources of off-policy data given by  replay buffers or premature episode truncations, cannot be easily corrected with importance sampling.

Most of the algorithm, in practice, do not correct off-policy distribution. We refer to this class of algorithms as \textsl{semi-gradient} (term introduced by \cite{imani_off-policy_2018} in the context of policy-gradient algorithms). \cite{imani_off-policy_2018} showed that using off-policy distributions without corrections can result in a poor convergence, as the distribution shift results in an irreducible bias of the gradient estimator.
Many recent techniques aim to correct the sampling process to match the on-policy distribution using sophisticated versions of importance sampling corrections or working with surrogate objective. They will be discussed in Section~\ref{sec:related-work}. Our work, however, follows an alternative path by \textsl{overcoming the need of using on-policy data}.
